Vision-Grounded Semantic Learning and Alignment for Scalable Multilingual Text-Based Person Retrieval

Multilingual Text-Based Person Retrieval (TBPR) aims to retrieve individuals with texts in multiple languages. Despite its practical importance, it has been overlooked by existing research, which mainly focuses on English-only retrieval. The only prior attempt at multilingual TBPR suffers from (1) the absence of a large-scale, multilingual pretraining dataset and (2) a suboptimal model architecture for multilingual text encoding and cross-modal alignment, which employs a shared encoder that overlooks linguistic heterogeneity and relies on English as a pivot for cross-modal alignment, introducing English-centric bias. For this, we contribute MultiPedes, the first large-scale, pedestrian-centric multilingual pretraining dataset. It contains 10 million image-text pairs across four languages, constructed by a multilingual quality-aware data construction pipeline. We also propose ViSeLA (Vision-grounded Semantic Learning and Alignment), a novel framework featuring: (1) a semantic-aware multilingual learning module that extends the mixture-of-experts architecture by routing language-invariant semantics to specialized experts for improved multilingual feature learning; and (2) a vision-grounded cross-modal alignment module that employs a semantic probe to capture fine-grained semantics across modalities, enabling direct cross-modal alignment without relying on a pivot language. Extensive experiments on both multilingual and English-only TBPR datasets demonstrate the effectiveness of ViSeLA. The dataset and code are available at https://github.com/Flame-Chasers/ViSeLA

==> tables/table5.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Ablation study on the key component of proposed multilingual quality-aware data construction
pipeline. Results are averaged on CUHK-PEDES.}
    \label{tab:ablation_data}

    \renewcommand\arraystretch{1.2}
    \setlength{\extrarowheight}{3pt}

    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|cccc}
        \hline\thickhline
        \rowcolor{lightgray}   
        No. & Data Construction Pipeline & R@1 & R@5 & R@10 & mAP \\
        \hline\hline
        1 & w/o Consensus-Guided Filtering & 76.57 & 89.42 & 93.02 & 69.16 \\
        \rowcolor[HTML]{D7F6FF}
        2 & w Consensus-Guided Filtering & \textbf{77.94} & \textbf{90.94} & \textbf{94.29} & \textbf{70.16} \\
        \hline\thickhline
    \end{tabular}%
    }
\end{table}
